Nominal Algebraic-Coalgebraic Data Types, with Applications to Infinitary Lambda-Calculi

Ten years ago, it was shown that nominal techniques can be used to design coalgebraic data types with variable binding, so that alpha-equivalence classes of infinitary terms are directly endowed with a corecursion principle. We introduce "mixed" binding signatures, as well as the corresponding type of mixed inductive-coinductive terms. We extend the aforementioned work to this setting. In particular, this allows for a nominal description of the sets Lambda_abc of abc-infinitary lambda-terms (for a, b, c in {0,1}) and of capture-avoiding substitution on alpha-equivalence classes of such terms.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{Alexis Saurin (Editor): Fixed Points\\ 
in Computer Science 2024 (FICS 2024).\\
EPTCS 435, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.435.5}{10.4204/EPTCS.435.5}}
\pdfoutput=1

